Efficient Compilation to Event-Driven Task Programs

As illustrated by the emergence of a class of new languages and runtimes, it is expected that a large portion of the programs to run on extreme scale computers will need to be written as graphs of event-driven tasks (EDTs). EDT runtime systems, which schedule such collections of tasks, enable more concurrency than traditional runtimes by reducing the amount of inter-task synchronization, improving dynamic load balancing and making more operations asynchronous. We present an efficient technique to generate such task graphs from a polyhedral representation of a program, both in terms of compilation time and asymptotic execution time. Task dependences become materialized in different forms, depending upon the synchronization model available with the targeted runtime. We explore the different ways of programming EDTs using each synchronization model, and identify important sources of overhead associated with them. We evaluate these programming schemes according to the cost they entail in terms of sequential start-up, in-flight task management, space used for synchronization objects, and garbage collection of these objects. While our implementation and evaluation take place in a polyhedral compiler, the presented overhead cost analysis is useful in the more general context of automatic code generation.

==> autodec.tex <==
\section{Enabling optimal overheads} \label{sec:autodec}
Sequential overhead results from the inability to determine, for a given
successor task with multiple predecessors, a unique predecessor that can set up
the successor task (let us call such task the successor's creator). 

As we saw in Section \ref{sec:tags}, we assume that there is no general way to
resolve this statically. 
We propose a dynamic resolution based on counted dependences, which does not
introduce sequentializing dependences. 
In our proposed dynamic resolution, the first task to be able to decrement a
successor task's counter becomes its creator. 
We call such decrement with automatic creation an ``autodec'' operation. 

Creation of a unique counted dependence - and hence a unique successor task - is
ensured through the use of an atomic compare-and-swap operation, as detailed in
Algorithm \ref{algo:autodec}. 
Atomicity deals with the presumably rare case when two predecessors complete at
the exact same time. 

At a high level, running each task is equivalent to calling a function $f$ with
parameters $p$: $f(p)$. 
A programmatic scheme for using autodecs relies on the definition of three
helper functions for each $f$: 
\begin{itemize}
\item a function $f\_count(p)$ that counts the number of input dependences to
  $f(p)$, 
\item a function $f\_pack(p)$ that sets up the counted dependence, including the
  arguments to pass to $f(p)$, and 
\item an injective function $f\_rank(p)$ that maps $p$ to a unique identifier.
 The set of all $f\_rank()$ functions must be such that each pair $(f,p)$ maps to
 a unique identifier. 
 In our framework, $f\_rank(p)$ returns an integer, which allows us to store
 counted dependences in either an array or a map. 
\end{itemize}

\begin{algorithm}[h]
\KwData{f: successor task function descriptor\;
        p: set of task parameters to the successor task\;}
\Begin{
 rank = f\_rank(p)\;
 countedDep cdep = counted\_deps[rank]\;
 \eIf{cdep is initialized}
     {decrement cdep\;}
     {
       count  = f\_count(p)\;
       \tcp*[r]{autodec is called by a predecessor}
       assert count!=0\; 
       new\_counted\_dep = f\_pack(p, count)\;
       swapped = compare\_and\_swap(counted\_deps[rank], null, new\_counted\_dep)\;
       \eIf{swapped}
           {decrement new\_counted\_dep\;}
           {
            decrement counted\_deps[rank]\;
            delete new\_dep\;
           }
      }
}
\caption{{\em autodec} operation pseudo-code} \label{algo:autodec}
\end{algorithm}

As a result, only tasks that don't have a predecessor need to be scheduled by
the master task (no sequential start-up overhead). 
The tasks that have predecessors are scheduled upon the first completion of one
of their predecessors, resulting in an $O(r)$ in-flight scheduling overhead. 

An $O(r)$ spatial overhead can be obtained by storing the counted dependences in
a map (for instance a hash map), at the price of slightly heavier
synchronization mechanisms. 

Consider the case where the set of tasks without predecessors is unknown. 
Since we know the set of predecessors for each task, one solution would be to
identify this set by scanning all the tasks and collecting the ones with zero
predecessors. Unfortunately, this would entail an $O(n)$ sequential overhead in
the best case. 
To avoid this need, we introduce the ``preschedule'' operation, in which a
 counted dependence is atomically initialized - as in autodecs - but not
 decremented. 
The fact that the same mechanism is used by autodec and preschedule operations
guarantees that no counted dependence will be created more than once, and that
no task will be executed more than once. 
Hence, the order in which the master task preschedules tasks and tasks
auto-decrement their successors does not matter, and preschedule operations can
execute concurrently with the tasks, resulting in a $O(1)$ sequential start-up
overhead. 

In the context of automatic parallelization to task graphs using the polyhedral
model, there is a straightforward automatic method for determining the set of
tasks without predecessors. 
Unfortunately, this method is not generally tractable, but there is a tractable
method for computing a slight over-approximation of the set. 
This slightly over-approximated set is prescheduled by the host, and the tasks
that are in this set but have predecessors may be initialized by either the
master task or one of the task's predecessors, depending upon which one executes
its initialization first. 

Overhead for autodec-based systems are summarized in Table 
\ref{table:autodec-cplexities} for the cases when the set of sources is known
(``w/ src'' row) and unknown (``w/o src'' row). 
\begin{table}
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline
 ~          & Sequential & Spatial  & In-flight & Garb. coll. \\ \hline
w/o src &  $O(1)$    &  $O(n)$  &   $O(n)$  & $O(1)$ \\ \hline
w/ src  &  $O(1)$    &  $O(r)$  &   $O(r)$  & $O(1)$ \\ \hline
\end{tabular}
\end{center}
\caption{Overheads associated with autodecs} \label{table:autodec-cplexities}
\end{table}

A similar synchronization combined with task initialization could be implemented
on top of tags using method 1, using an ``auto-put'' operation, through which
the first predecessor to a task also sets up the task. Unfortunately, this
method would suffer from a higher spatial overhead ($O(r^2)$), since one tag is
associated with each dependence. 

We have given thought to other tag-based ways of implementing similar
synchronization mechanism, for instance using method 2.
But, in our view, they all boil down to re-implementing autodecs based on counted
dependences, or perhaps slight variants of them. 

\subsection{Implementation details}
We implemented this system on top of the SWARM runtime for x86 multi-core
architectures. 
We intend to implement support for autodecs in OCR as well. 

The convention between our code generator and the runtime is as follows, for a
task identified by function call $f(p)$: 
\begin{itemize}
\item The function counting the task's input dependences is named
  $f\_count(p)$.
  Our code generator supports two implementations: one uses a loop that scans
  them and increments a counter by one for each of them, and the other one uses
  a direct analytical model of the number of predecessor tasks as a function of
  $p$. 
\item The function initializing the counted dependence parameters is named 
  $f\_pack$.\footnote{Initialization typically includes the packaging of $p$ into
  data structures associated with $f(p)$. 
  The details of how parameters are passed to the tasks and their helper
  functions is defined by the underlying runtime API, and are not discussed
  here.}
\item The function associating $f(p)$ with a unique integer identifier is named
  $f\_rank$. 
\end{itemize}

\subsection{Distributed case} \label{ssec:distributed}
The presented system is straightforwardly extensible to distributed
computations if the mapping from counted dependences to compute nodes is
determined and known to all the nodes when the counted dependence is
initialized. 
As long as all the atomic operation is performed on the same node, there are no
race conditions. 


==> counted.tex <==
\section{Counted dependences} \label{sec:counted}
Counted dependences have similarities with both prescribed synchronizations and
tags.
Like prescribed synchronization, they require a task to initialize them. 
Programmatically, a counted dependence represents the number of unsatisfied
input dependences of a successor task. 
It is decremented by each predecessor of the task.
Without further synchronization, counted dependences have an $O(n^2)$
sequential overhead as prescribed synchronizations if the input dependences need
to be enumerated, or $O(n.d)$ if there exists an analytic function that computes
them in time $d$.
Such functions are available in the context of automatic generation based on the
polyhedral model, and the computational complexity of these functions is bounded
by a (potentially large) constant. 

The fact that the program start with $n$ tasks to schedule implies an in-flight
task overhead of $O(n)$.
Only one counted dependence is required for each task, giving a spatial overhead
of $O(n)$. 
Garbage collection of the counted dependence associated with each task can be
performed as soon as the task starts. 

Overheads associated with programmatic use of the three task synchronization
constructs are summarized in Table \ref{table:overhead-summary}. 
Method 2 of the tags system was implemented independently
\cite{anonymous}. 
This method uses tags with SWARM and CnC, and imports a tags construct to OCR.
\begin{table}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
 ~         & Sequential & Spatial  & In-flight & Garb. coll. \\ \hline
Prescribed & $O(n^2)$   & $O(n^2)$ & $O(n)$    & $O(n)$        \\ \hline
Tags 1     & $O(1)$     & $O(n^2)$ & $O(n)$    & $O(1)$        \\ \hline
Tags 2     & $O(1)$     & $O(n)$   & $O(n)$    & $O(n)$        \\ \hline
Counted    & $O(n.d)$   & $O(n)$   & $O(n)$    & $O(1)$        \\ \hline
\end{tabular}
\end{center}
\caption{Overheads associated with task graph synchronization
  modes}\label{table:overhead-summary}
\end{table}

The best methods are tags with method 2, followed by counted dependences. 
An ideal task graph runtime scheme would have constant sequential and garbage
collection overhead. 
The set of useful in-flight scheduled tasks should be the ones that are
ready to run, i.e., the ones whose input dependences are satisfied, plus the
ones that are already running. 
Let us call $r$ the maximum number of such tasks in any execution of the task
graph.
Having less than $r$ in-flight tasks reduces parallelism and is hence not
desirable.
An ideal task graph runtime scheme would have $O(r)$ in-flight task overhead and,
accordingly, an $O(r)$ spatial overhead. 

In the next section, we introduce a new synchronization mechanism that extends
counted dependences in order to reduce sequential, spatial and in-flight
overheads down to their optimal amounts. 


==> tags.tex <==
\section{Tag-based synchronization} \label{sec:tags}
With tags, a predecessor and its successor tasks synchronize through a tag that
represents the completion of the predecessor task to the successor task. 
A tag is notionally a key in an associative table.
The predecessor signifies its completion by putting the tag in the table. 
The successor can wait for tags to be available in the table by getting the
tag. 
Control returns to the task whenever all the tags for which a ``get'' was issued
have been put in the table. 
To avoid deadlocks, gets are typically asynchronous.
The SWARM runtime, for example, de-schedules a task that issues a ``get'' and
queues it to the tag.
When a tag is put, all the tasks that are queued to the tag are re-scheduled. 

We have found two methods for programmatically using tags as a means of
inter-task synchronization. 
\begin{enumerate}
\item [1.] In the first method, a tag straightforwardly represents a dependence,
  i.e., a relationship between two tasks. 
  Predecessor tasks put one tag in the table for each successor they have, and
  successor tasks get one tag for each predecessor they have. 
\item [2.] In the second method, one tag is associated with one task.
  A task that has successors puts a tag that signifies that it has completed. 
  Its successors all get the same tag from the table. 
\end{enumerate}

The main clear advantage of these methods, as compared to prescribed
synchronization methods, is that they have no sequential scheduling overhead,
since all tasks can be started in parallel, virtually at any point in time. 

The cost of storing synchronization objects (spatial overhead) differentiates
both methods. 
It is $O(n^2)$ for Method 1 (one tag per dependence), and $O(n)$ for Method 2
(one tag per task). 
However, Method 1 has an advantage in terms of garbage-collection of its tags,
since a tag can be disposed of as soon as its unique ``get'' has executed. 
The SWARM runtime offers one-use tags, where the disposal of a tag is performed
by the runtime after a ``get'' was done on the tag. 
In Method 2, without further sequentializing synchronization, successor tasks
don't know whether they are the last task to ``get'' the tag. 
Hence the tag objects can only be disposed once a post-dominator of the task
graph has started, or when the entire task graph has completed. 

To estimate the impact of spatial overhead combined with garbage collection, as
present in Method 1, we implemented Method 1 on top of the SWARM runtime. 
We generated a parallel application with above a million (1309442 to be precise)
very small tasks, and with transitively redundant dependences in order to get as
close as reasonable to an $n^2$ occupancy. 
We ran the experiment on a 24-core Xeon E5-2620 running at 2.00GHz with 32Gb
RAM running Linux Ubuntu 12.04, and we monitored memory usage.
The program eventually used up all the RAM and was killed by the Linux kernel. 
This means that an $O(n^2)$ space overhead is not acceptable at Exascale, since
it is already not viable at Gigascale. 

In terms of in-flight task overhead, a straightforward implementation of both
methods consists in starting all the tasks upfront and letting them synchronize
with each other.
To reduce the number of tasks to be managed by the scheduler simultaneously,
tasks should be scheduled by their predecessors. 
The tightest bound on the number of in-flight tasks is obtained when each task
is scheduled by one of its predecessors. 
In this case, the number of in-flight scheduled tasks is exactly the number of
tasks that are ready to run. 
The main obstacle to achieving this appears again with tasks that have more than
one predecessor, in which case one of the predecessors must be chosen to
schedule the successor task. 
This cannot be performed dynamically using tags without introducing
sequentializing synchronizations. 

Methods for statically electing a task within a set of tasks are available in
the context of automatic parallelization using the polyhedral model. 
For any given successor task, the method consists in considering a total order
among the set of predecessor tasks, and defining the task that minimizes the order
 \cite{feautrier88parametric} as the one that schedules the successor task. 
Unfortunately, except for simple cases, the computation of such a minimum
doesn't scale well with the maximum number of nested loops in the program,
leading to potentially intractable execution times of the automatic
parallelization tool. 
Additionally, this solution is specific to the polyhedral model, as opposed to
the more general problem of programmatically using task-based runtimes.

Hence, when using tag synchronization, the straightforward solution is the only
one generally available, with a $O(n)$ in-flight task overhead.

